On the Cryptographic Structure Required for Verifying Qubits

Classically testing for the presence of anti-commuting operators on a quantum device is a critical tool underpinning recent progress in classical verification of quantum computation. While such tests can be based on cryptographic assumptions, known constructions rely on highly structured assumptions, e.g. trapdoor claw-free functions. In this work, we seek to explain this state of affairs by constructing strong cryptography from (certain forms of) classical tests of anti-commutation. In particular, we formulate the notion of a test of non-commutation (ToNC), an interactive protocol between a quantum prover and classical verifier in which the prover's final-round response is obtained by measuring one of two binary observables $P_0,P_1$ depending on the verifier's challenge bit $c$. We prove that, for a broad range of parameters, ToNC implies classical-communication key agreement (KA), and ToNC combined with one-way functions implies oblivious transfer (OT). Along the way, we develop tools for and provide the first known results on hardness amplification for post-quantum KA and OT, where communication is classical but adversaries may be quantum. In particular, we prove the following results of independent interest. - Post-quantum hard-core measure theorem: For any efficiently sampleable high-min-entropy distribution $D$ over pairs $(x,b)$ such that quantum circuits have advantage at most $\delta$ in predicting $b$ from $x$, there exists a sub-distribution $M\preceq D$ of density $(1-\delta)$ on which $b$ is nearly optimally quantum-hard to predict. - Post-quantum interactive XOR lemma: Given any classically-interactive protocol, if quantum adversaries have advantage at most $\delta$ in guessing a private challenger bit $b$, then two sequential repetitions reduce the advantage for predicting the XOR of the challenger bits $b_1\oplus b_2$ to at most $\delta^2+\rm{negl}(\lambda)$.

==> james-macros.tex <==
\newcommand{\textdef}[1]{\textnormal{\textsf{#1}}}

\RequirePackage{aliascnt}

\newcommand{\newsharedtheorem}[3]{%
  \newaliascnt{#1}{theorem}%
  \newtheorem{#1}[#1]{#2}%
  \aliascntresetthe{#1}%
  \crefname{#1}{#2}{#3}%
  \Crefname{#1}{#2}{#3}%
}

\ifsubmission

\newsharedtheorem{axiom}{Axiom}{Axioms}
\newsharedtheorem{physicsaxiom}{Physics Axiom}{Physics Axioms}
\newsharedtheorem{importedtheorem}{Imported Theorem}{Imported Theorems}
\newsharedtheorem{importedlemma}{Imported Lemma}{Imported Lemmas}
\newsharedtheorem{informaltheorem}{Informal Theorem}{Informal Theorems}
\newsharedtheorem{physicstheorem}{Physical Theorem}{Physical Theorems}
\let\claim\relax
\newsharedtheorem{claim}{Claim}{Claims}
\newsharedtheorem{subclaim}{SubClaim}{SubClaims}
\newsharedtheorem{fact}{Fact}{Facts}
\newsharedtheorem{construction}{Construction}{Constructions}
\crefname{theorem}{Theorem}{Theorems}
\Crefname{theorem}{Theorem}{Theorems}
\crefname{proposition}{Proposition}{Propositions}
\Crefname{proposition}{Proposition}{Propositions}
\crefname{subsubclaim}{SubSubClaim}{SubSubClaims}
\Crefname{subsubclaim}{SubSubClaim}{SubSubClaims}
\crefname{lemma}{Lemma}{Lemmas}
\Crefname{lemma}{Lemma}{Lemmas}
\crefname{conjecture}{Conjecture}{Conjectures}
\Crefname{conjecture}{Conjecture}{Conjectures}
\crefname{corollary}{Corollary}{Corollaries}
\Crefname{corollary}{Corollary}{Corollaries}
\crefname{property}{Property}{Properties}
\Crefname{property}{Property}{Properties}

\theoremstyle{definition}

\newsharedtheorem{assumption}{Assumption}{Assumptions}
\newsharedtheorem{notation}{Notation}{Notations}
\crefname{definition}{Definition}{Definitions}
\Crefname{definition}{Definition}{Definitions}

\theoremstyle{remark}

\ifsubmission\else\newsharedtheorem{comment}{Comment}{Comments}\fi

\crefname{question}{Question}{Questions}
\Crefname{question}{Question}{Questions}
\crefname{remark}{Remark}{Remarks}
\Crefname{remark}{Remark}{Remarks}
\crefname{comment}{Comment}{Comments}
\Crefname{comment}{Comment}{Comments}
\crefname{step}{Step}{Steps}
\Crefname{step}{Step}{Steps}

\else

\newtheorem{theorem}{Theorem}[section]
\crefname{theorem}{Theorem}{Theorems}
\Crefname{theorem}{Theorem}{Theorems}

\newsharedtheorem{axiom}{Axiom}{Axioms}
\newsharedtheorem{physicsaxiom}{Physics Axiom}{Physics Axioms}
\newsharedtheorem{importedtheorem}{Imported Theorem}{Imported Theorems}
\newsharedtheorem{importedlemma}{Imported Lemma}{Imported Lemmas}
\newsharedtheorem{informaltheorem}{Informal Theorem}{Informal Theorems}
\newsharedtheorem{physicstheorem}{Physical Theorem}{Physical Theorems}
\newsharedtheorem{proposition}{Proposition}{Propositions}
\newsharedtheorem{claim}{Claim}{Claims}
\newsharedtheorem{subclaim}{SubClaim}{SubClaims}
\newsharedtheorem{subsubclaim}{SubSubClaim}{SubSubClaims}
\newsharedtheorem{lemma}{Lemma}{Lemmas}
\newtheorem{conjecture}{Conjecture}
\crefname{conjecture}{Conjecture}{Conjectures}
\Crefname{conjecture}{Conjecture}{Conjectures}
\newsharedtheorem{corollary}{Corollary}{Corollaries}
\newsharedtheorem{fact}{Fact}{Facts}
\newsharedtheorem{property}{Property}{Properties}
\newsharedtheorem{construction}{Construction}{Constructions}
\newsharedtheorem{definition}{Definition}{Definitions}
\newsharedtheorem{remark}{Remark}{Remarks}

\theoremstyle{definition}
\newsharedtheorem{assumption}{Assumption}{Assumptions}
\newsharedtheorem{notation}{Notation}{Notations}

\theoremstyle{remark}
\newsharedtheorem{question}{Question}{Questions}
%\newtheorem{comment}[theorem]{Comment}

\crefname{comment}{Comment}{Comments}
\Crefname{comment}{Comment}{Comments}
\crefname{step}{Step}{Steps}
\Crefname{step}{Step}{Steps}

\newsharedtheorem{example}{Example}{Examples}
\fi


%%%%%%%%%%%%%%%%% SOME BASIC DEFINITIONS %%%%%%%%%%%%%%%%%%

%Security Parameter

%\newcommand{\secp}{\lambda}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Calligraphic and blackboard type letters.

\def\cA{{\cal A}}
\def\cB{{\cal B}}
\def\cC{{\cal C}}
\def\cD{{\cal D}}
\def\cE{{\cal E}}
\def\cF{{\cal F}}
\def\cG{{\cal G}}
\def\cH{{\cal H}}
\def\cI{{\cal I}}
\def\cJ{{\cal J}}
\def\cK{{\cal K}}
\def\cL{{\cal L}}
\def\cM{{\cal M}}
\def\cN{{\cal N}}
\def\cO{{\cal O}}
\def\cP{{\cal P}}
\def\cQ{{\cal Q}}
\def\cR{{\cal R}}
\def\cS{{\cal S}}
\def\cT{{\cal T}}
\def\cU{{\cal U}}
\def\cV{{\cal V}}
\def\cW{{\cal W}}
\def\cX{{\cal X}}
\def\cY{{\cal Y}}
\def\cZ{{\cal Z}}


\def\regA{{\cal A}}
\def\regB{{\cal B}}
\def\regC{{\cal C}}
\def\regD{{\cal D}}
\def\regE{{\cal E}}
\def\regF{{\cal F}}
\def\regG{{\cal G}}
\def\regH{{\cal H}}
\def\regI{{\cal I}}
\def\regJ{{\cal J}}
\def\regK{{\cal K}}
\def\regL{{\cal L}}
\def\regM{{\cal M}}
\def\regN{{\cal N}}
\def\regO{{\cal O}}
\def\regP{{\cal P}}
\def\regQ{{\cal Q}}
\def\regR{{\cal R}}
\def\regS{{\cal S}}
\def\regT{{\cal T}}
\def\regU{{\cal U}}
\def\regV{{\cal V}}
\def\regW{{\cal W}}
\def\regX{{\cal X}}
\def\regY{{\cal Y}}
\def\regZ{{\cal Z}}


\newcommand{\sA}{\mathsf{A}}
\newcommand{\sB}{\mathsf{B}}
\newcommand{\sC}{\mathsf{C}}
\newcommand{\sD}{\mathsf{D}}
\newcommand{\sE}{\mathsf{E}}
\newcommand{\sF}{\mathsf{F}}
\newcommand{\sG}{\mathsf{G}}
\newcommand{\sH}{\mathsf{H}}
\newcommand{\sI}{\mathsf{I}}
\newcommand{\sJ}{\mathsf{J}}
\newcommand{\sK}{\mathsf{K}}
\newcommand{\sL}{\mathsf{L}}
\newcommand{\sM}{\mathsf{M}}
\newcommand{\sN}{\mathsf{N}}
\newcommand{\sO}{\mathsf{O}}
\newcommand{\sP}{\mathsf{P}}
\newcommand{\sQ}{\mathsf{Q}}
\newcommand{\sR}{\mathsf{R}}
\newcommand{\sS}{\mathsf{S}}
\newcommand{\sT}{\mathsf{T}}
\newcommand{\sU}{\mathsf{U}}
\newcommand{\sV}{\mathsf{V}}
\newcommand{\sW}{\mathsf{W}}
\newcommand{\sX}{\mathsf{X}}
\newcommand{\sY}{\mathsf{Y}}
\newcommand{\sZ}{\mathsf{Z}}

%%%%%%%%%%%%%%%%%

% Blackboard fonts

\def\bbC{{\mathbb C}}
\def\bbE{{\mathbb E}}
\def\bbF{{\mathbb F}}
\def\bbG{{\mathbb G}}
\def\bbI{{\mathbb I}}
\def\bbM{{\mathbb M}}
\def\bbN{{\mathbb N}}
\def\bbQ{{\mathbb Q}}
\def\bbR{{\mathbb R}}
\def\bbV{{\mathbb V}}
\def\bbZ{{\mathbb Z}}

\newcommand{\bbma}{\mathbbm{a}}
\newcommand{\bbmb}{\mathbbm{b}}
\newcommand{\bbmp}{\mathbbm{p}}
\newcommand{\bbmu}{\mathbbm{u}}
\newcommand{\bbmv}{\mathbbm{v}}
\newcommand{\bbmx}{\mathbbm{x}}
\newcommand{\bbmy}{\mathbbm{y}}
\newcommand{\bbmz}{\mathbbm{z}}

%%%%%%%%%%%%%%%

% bold fonts
\newcommand{\ba}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\bd}{\mathbf{d}}
\newcommand{\be}{\mathbf{e}}
%\newcommand{\bf}{\mathbf{f}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\bh}{\mathbf{h}}
\newcommand{\bi}{\mathbf{i}}
\newcommand{\bj}{\mathbf{j}}
\newcommand{\bk}{\mathbf{k}}
\newcommand{\bl}{\mathbf{l}}
%\newcommand{\bm}{\mathbf{m}}
\newcommand{\bn}{\mathbf{n}}
\newcommand{\bo}{\mathbf{o}}
\newcommand{\bp}{\mathbf{p}}
\newcommand{\bq}{\mathbf{q}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\bt}{\mathbf{t}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}


\newcommand{\bA}{\mathbf{A}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bX}{\mathbf{X}}


\newcommand{\brho}{\boldsymbol{\rho}}
\newcommand{\bsigma}{\boldsymbol{\sigma}}
\newcommand{\btau}{\boldsymbol{\tau}}
\newcommand{\bpsi}{\boldsymbol{\psi}}
\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\bTheta}{\boldsymbol{\Theta}}
\newcommand{\bDelta}{\boldsymbol{\Delta}}


%%%%%%%%%%%%%%%
% Algebra %
%\newcommand{\F}{\bbF}
\newcommand{\Zq}{\bbZ_q}
\newcommand{\Z}{\bbZ}
\newcommand{\N}{\bbN}
\newcommand{\xor}{\oplus}
\newcommand{\tensor}{\otimes}
%\newcommand{\transp}{\top}

%%%%%%%%%%%%%%%
% Analysis %
\newcommand{\R}{\bbR}

%%%%%%%%%%%%%%%
% Asymptotics %

\def\poly{{\rm poly}}
\def\polylog{{\rm polylog}}
\def\polyloglog{{\rm polyloglog}}
\def\negl{{\rm negl}}

%%%%%%%%%% Automata %%%%%%%%%%
\newcommand{\qinitial}{q_0}
\newcommand{\qaccept}{q_{\mathsf{acc}}}
\newcommand{\qreject}{q_{\mathsf{rej}}}

%%%%%%%%%%%%%%% Crypto %%%%%%%%%%

% Miscellaneous
\newcommand{\pk}{\mathsf{pk}}
\newcommand{\sk}{\mathsf{sk}}
\newcommand{\dist}{\mathsf{dist}}
\newcommand{\KeyGen}{\mathsf{KeyGen}}
\newcommand{\Setup}{\mathsf{Setup}}
\newcommand{\Commit}{\mathsf{Commit}}
%\newcommand{\com}{\mathsf{com}}
%\newcommand{\Com}{\mathsf{Com}}
\newcommand{\decom}{\mathsf{decom}}
\newcommand{\Sim}{\mathsf{Sim}}
\newcommand{\Sign}{\mathsf{Sign}}
\newcommand{\Enc}{\mathsf{Enc}}
%\newcommand{\Dec}{\mathsf{Dec}}
\newcommand{\Mark}{\mathsf{Mark}}
\newcommand{\Verify}{\mathsf{Verify}}
\newcommand{\iO}{\mathsf{i}\mathcal{O}}
\newcommand{\diO}{\mathsf{di}\mathcal{O}}
\newcommand{\clenc}{\mathsf{ClEnc}}
\newcommand{\nizk}{\mathsf{NIZK}}
\newcommand{\ct}{\mathsf{ct}}



% Oblivious RAM
\newcommand{\OMem}{\mathsf{OMem}}
\newcommand{\OProg}{\mathsf{OProg}}
\newcommand{\ReadWrite}{\mathsf{ReadWrite}}
\newcommand{\Read}{\mathsf{Read}}
\newcommand{\Write}{\mathsf{Write}}
\newcommand{\OSample}{\mathsf{OSample}}
\newcommand{\OEncode}{\mathsf{OEncode}}
\newcommand{\OAccess}{\mathsf{OAccess}}
\newcommand{\Access}{\mathsf{Access}}


% puncturable PRF macros
\newcommand{\PPRF}{\mathcal{PPRF}}
\newcommand{\Eval}{\mathsf{Eval}}
\newcommand{\Puncture}{\mathsf{Puncture}}
\newcommand{\PuncEval}{\mathsf{PuncEval}}
\newcommand{\constrain}{\mathsf{Constrain}}
\newcommand{\punc}[2] { #1\{#2\}  }		% puncture, e.g. \punc{K}{C} ->
% K{C}

% Randomized Encoding Scheme
\newcommand{\RE}{\mathcal{RE}}

%%%%%%%%%%%%%%%%

% Probability and statistics

\let\E\relax
\DeclareMathOperator*{\E}{\mathbb{E}}
%\renewcommand{\E}{\expectation}
\DeclareMathOperator*{\Var}{\mathrm{Var}}
\newcommand{\rv}[1]{\mathbf{#1}} % random variable font
%\newcommand{\samp}{\gets}
\newcommand{\dtv}{d_{\mathsf{TV}}}
\newcommand{\MutInf}{\textbf{I}}
\newcommand{\Supp}{\mathrm{Supp}}
\newcommand{\probto}{\stackrel{\$}{\to}}

\newcommand{\BuildOut}{\mathsf{BuildOut}}
\newcommand{\Found}{\mathsf{Found}}
\newcommand{\Bad}{\mathsf{Bad}}
\newcommand{\qQthree}{q_{\mathsf{Q3}}}
\newcommand{\rQthree}{r_{\mathsf{Q3}}}





%%%%%%%%%%%%%%%%%

% Set Theory
\newcommand{\union}{\cup}
\newcommand{\intersect}{\cap}
\newcommand{\disjunion}{\sqcup}
\newcommand{\Func}[2]{\mathrm{Func}(#1, #2)}
\newcommand{\compose}{\circ}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\Pow}{\cP}
\newcommand{\injto}{\hookrightarrow}

%%%%%%%%%%%%%%%%%

% Other short-hands

\newcommand{\binset}{\{0,1\}}
%\newcommand{\pmone}{\{-1, 1\}}
\newcommand{\eqdef}{\stackrel{\mathsf{def}}{=}}


%%%%%%%%%%%%%%%%%

% Random commands

\newcommand{\PRFGen}{\mathsf{PRFGen}}
\newcommand{\domain}{\binset^{n}}
\newcommand{\range}{\binset^{m}}
\newcommand{\Test}{\mathsf{Test}}
\newcommand{\Init}{\mathsf{Init}}
% % %
\newcommand{\pe}{\cP\cE}

%%%%%%%%%%%%%%%%%%

% Complexity

\newcommand{\TIME}{\mathsf{TIME}}
\newcommand{\NTIME}{\mathsf{NTIME}}
\newcommand{\SPACE}{\mathsf{SPACE}}
\newcommand{\TISP}{\mathsf{TISP}}

\newcommand{\Time}{\mathsf{Time}} 

\newcommand{\Space}{\mathsf{Space}}
\newcommand{\ioBPP}{\mathsf{io}\text{-}\mathsf{BPP}}
\renewcommand{\P}{\mathsf{P}}
\newcommand{\PSPACE}{\mathsf{PSPACE}}
\newcommand{\EXP}{\mathsf{EXP}}
\newcommand{\NEXP}{\mathsf{NEXP}}
\newcommand{\NP}{\mathsf{NP}}
\newcommand{\PCP}{\mathsf{PCP}}
\newcommand{\IP}{\mathsf{IP}}
\newcommand{\MIP}{\mathsf{MIP}}
\newcommand{\FP}{\mathsf{FP}}
\newcommand{\Prampoly}{\mathsf{P}_{\mathsf{RAM}}/\mathsf{poly}}
\newcommand{\Erampoly}{\mathsf{E}_{\mathsf{RAM}}/\mathsf{poly}}

%%%%%%%%%%%%%%%%

% Miscellaneous

\newcommand{\Gen}{\mathsf{Gen}}
\newcommand{\Present}{\mathsf{Present}}
\newcommand{\Extract}{\mathsf{Extract}}
\newcommand{\Spl}{\mathsf{Spl}}

\newcommand{\mk}{\mathsf{mk}}
\newcommand{\ek}{\mathsf{ek}}
\newcommand{\vk}{\mathsf{vk}}
\newcommand{\aux}{\mathsf{aux}}
\DeclareMathOperator{\Id}{Id}

%%%%%%%%%%%%%%%%

% Project-Specific

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


% \newcommand{\rank}{\mathsf{rank}}

%indicator vector map
%\newcommand{\ind}{\mathsf{Ind}} 

\newcommand{\bracket}[2]{\mbox{$\Braket { #1 | #2 }$}}

\DeclareMathOperator*{\expect}{\mathbf{E}}

%%%%%%%%%%%%%%%%

% Quantum

% using this for partial trace
\newcommand{\CM}{\mathsf{C+M}}
\newcommand{\dst}{\mathsf{dist}}
\newcommand{\identity}{\mathbb{I}}


% Proof Notations
\newcommand{\Hyb}{\mathsf{Hyb}}


% Actions
\newcommand{\uniformsample}{\overset{\$}{\gets}}



% Protocol environment

\newcommand{\proref}[1]{Protocol~\protect\ref{#1}}

\newenvironment{boxfig}[2]{\begin{figure}[#1]\fbox{
    \begin{minipage}{\linewidth}
    \vspace{0.2em}\makebox[0.025\linewidth]{}    \begin{minipage}{0.95\linewidth}{{#2 }}
    \end{minipage}\vspace{0.2em}\end{minipage}}}{\end{figure}}

\newenvironment{boxedalgo}
  {\begin{center}\begin{boxedminipage}{0.95\textwidth}}
  {\end{boxedminipage}\end{center}}

\newcommand{\pprotocol}[4]{
\begin{boxfig}{h!}{
\begin{center}
\textbf{#1}
\end{center}
    {\footnotesize#4}
\vspace{0.2em} } \caption{\label{#3} #2}
\end{boxfig}
}

\newcommand{\protocol}[4]{
\pprotocol{#1}{#2}{#3}{#4} }

% Garbled circuits

\newcommand{\Garble}{\mathsf{Garble}}
\newcommand{\GEval}{\mathsf{GEval}}
\newcommand{\GSim}{\mathsf{GSim}}

\newcommand{\QGarble}{\mathsf{QGarble}}
\newcommand{\QGEval}{\mathsf{QGEval}}
\newcommand{\QGSim}{\mathsf{QGSim}}

\newcommand{\labset}{\overline{\mathsf{lab}}}
\newcommand{\labsimset}{\widetilde{\mathsf{lab}}}
\newcommand{\labenc}{\mathsf{LabEnc}}
\newcommand{\lab}{\mathsf{lab}}

% 2PC

\newcommand{\crs}{\mathsf{crs}}
\newcommand{\inp}{\mathsf{inp}}
\newcommand{\zero}{\mathsf{zero}}
\newcommand{\twopc}{\mathsf{2PC}}
\newcommand{\gen}{\mathsf{Gen}}
\newcommand{\out}{\mathsf{Ver}}
%\newcommand{\state}{\mathsf{st}}

% FHE

\newcommand{\QMFHE}{\mathsf{QMFHE}}




\newcommand{\zo}{\{0,1\}}
\newcommand{\view}{\mathsf{View}}
\newcommand{\fot}{\mathcal{F}_{\mathsf{OT}}}
\newcommand{\simu}{\mathsf{Sim}}
\newcommand{\commit}{\mathsf{commit}}
\newcommand{\reveal}{\mathsf{reveal}}
%\newcommand{\Open}{\mathsf{Open}}
%\newcommand{\Rec}{\mathsf{Rec}}
\newcommand{\Dist}{\mathsf{Dist}}
\newcommand{\weakot}{{\mathsf{weak}\text{-}\mathsf{OT}}}
\newcommand{\equivsim}{\mathcal{Q}}
\newcommand{\open}{\mathsf{open}}

\newcommand{\extcommit}{\mathsf{Ext.Commit}}
\newcommand{\extdecommit}{\mathsf{Ext.Decommit}}
\newcommand{\final}{\mathsf{final}}
\renewcommand{\partial}{\mathsf{partial}}

\newcommand{\abort}{\mathsf{abort}}
\newcommand{\comb}{\mathsf{comb}}

\newcommand{\eecommit}{\mathsf{EECommit}}
\newcommand{\eedecommit}{\mathsf{EEDecommit}}

\newcommand{\RO}{\mathsf{RO}}
\newcommand{\sid}{\mathsf{sid}}
\newcommand{\internal}{\mathsf{int}}
\newcommand{\ext}{\mathsf{ext}}

%\newcommand{\Ext}{\mathsf{Ext}}
\newcommand{\Equ}{\mathsf{Equ}}

\newcommand{\SimExt}{\mathsf{SimExt}}
\newcommand{\SimEqu}{\mathsf{SimEqu}}

\newcommand{\TD}{\mathsf{TD}}
\newcommand{\ptrace}{\mathsf{Tr}}



\newcommand{\simurecv}{{\simu_{\cR^*}}}
\newcommand{\simusendr}{{\simu_{\cS^*}}}
\newcommand{\simucomm}{{\simu_{\cC^*}}}
\newcommand{\malrecv}{{\cR^*}}
\newcommand{\malsender}{{\cS^*}}
\newcommand{\malcomm}{{\cC^*}}
\newcommand{\maldist}{{\cD^*}}
\newcommand{\simuextrac}{\simu_{\Ext}}
\newcommand{\simuequ}{\simu_{\Equ}}
\newcommand{\outsendr}{{\mathsf{OUT}_S}}
\newcommand{\outmalrecv}{{\brho_{\malrecv}}}
\newcommand{\owhadv}{{\cA_{O2H}}}
\newcommand{\owhadvb}{{\cB_{O2H}}}



\newcommand{\idealcom}{\cF_{\text{so-com}}}
\newcommand{\picom}{\Pi_{\text{so-com}}}
\newcommand{\puncrom}[1]{{#1}^\bot}

\newcommand{\simucrecv}{\simu_{Com,\cR^*}}
\newcommand{\simuccomm}{\simu_{Com,\cC^*}}

\newcommand{\idealot}{\cF_{\text{OT}}}
\newcommand{\idealottwor}{\cF_{\text{OT}}}
\newcommand{\piotfourhyb}{{\Pi_{\text{OT}}^{\idealcom}}}
\newcommand{\piotfourcomp}{{\Pi_{\text{OT}}^{\idealcom/\picom}}}

\newcommand{\malcommlamb}{{\cC^*_\secp}}
\newcommand{\malrecvlamb}{\cR^*_\secp}
\newcommand{\maldistlamb}{\cD^*_\secp}
\newcommand{\simurecvlamb}{{\simu_{\secp,\malrecvlamb}}}
\newcommand{\brholamb}{\brho_\secp}
\newcommand{\qlamb}{q_\secp}
\newcommand{\GF}{\mathsf{GF}}
\newcommand{\Exp}{\mathsf{Exp}}
\newcommand{\pr}{\mathsf{pr}}
\newcommand{\wt}{\mathsf{wt}}

\newcommand{\RCommit}{\mathsf{RCommit}}
\newcommand{\ROpen}{\mathsf{ROpen}}


\newcommand{\idealuccom}{\cF_{\text{com}}}
\newcommand{\piuccom}{\Pi_{\text{com}}}
\newcommand{\simro}{\Sim_{\mathsf{RO}}}

\newcommand{\nc}{\mathsf{nc}}


\newcommand{\rcv}{\mathsf{R}}
%\newcommand{\Adv}{\mathsf{Adv}}


\newcommand{\sendr}{\mathsf{S}}
\newcommand{\recv}{\mathsf{R}}
\newcommand{\OT}{\mathsf{OT}}
\newcommand{\EndSROT}{\mathsf{End}-\mathsf{S}-\mathsf{ROT}}
\newcommand{\EndRROT}{\mathsf{End}-\mathsf{R}-\mathsf{ROT}}
\newcommand{\SROT}{\mathsf{S}-\mathsf{ROT}}
\newcommand{\RROT}{\mathsf{R}-\mathsf{ROT}}

\newcommand{\maj}{\mathsf{maj}}
\newcommand{\simroco}{\Sim_{\mathsf{RO}}^{\mathsf{CO}}}


\newcommand{\Adva}{\mathsf{AdvA}}
\newcommand{\Advb}{\mathsf{AdvB}}
\newcommand{\Advc}{\mathsf{AdvC}}

\newcommand{\strq}{\bq}
%\newcommand{\msg}{\mathsf{msg}}
\newcommand{\ctl}{\mathsf{ctl}}
\newcommand{\chk}{\mathsf{chk}}
\newcommand{\PKE}{\mathsf{PKE}}
\newcommand{\NIZK}{\mathsf{NIZK}}
\newcommand{\Prove}{\mathsf{Prove}}
%\newcommand{\Ver}{\mathsf{Ver}}
\newcommand{\PRG}{\mathsf{PRG}}
\newcommand{\hk}{\mathsf{hk}}
\newcommand{\otp}{\mathsf{otp}}
\newcommand{\sd}{\mathsf{sd}}
\newcommand{\cm}{\mathsf{cm}}
%\newcommand{\hm}{\mathsf{hm}}
\newcommand{\ck}{\mathsf{ck}}
\newcommand{\hsh}{\mathsf{hsh}}
\newcommand{\ExtGen}{\mathsf{ExtGen}}
\newcommand{\Samp}{\mathsf{Samp}}
\newcommand{\ROT}{\mathsf{ROT}}
\newcommand{\CI}{\mathsf{CI}}
\newcommand{\CL}{\mathsf{CL}}
\newcommand{\QU}{\mathsf{QU}}
\newcommand{\ZKSS}{\mathsf{SS}}
\newcommand{\hw}{\mathsf{hw}}
\newcommand{\nonnegl}{\mathsf{non}\text{-}\mathsf{negl}}
\newcommand{\ots}{\mathsf{ots}}
\newcommand{\C}{\mathsf{C}}
\newcommand{\NC}{\mathsf{NC}}
\newcommand{\continue}{\mathsf{continue}}
\newcommand{\EQ}{\mathsf{EQ}}
\newcommand{\QMA}{\mathsf{QMA}}
\newcommand{\pre}{\mathsf{pre}}
\newcommand{\chck}{\mathsf{check}}
\newcommand{\post}{\mathsf{post}}
\newcommand{\NAND}{\mathsf{NAND}}
\newcommand{\co}{\mathsf{co}}
\newcommand{\spn}{\mathsf{span}}
\newcommand{\prep}{\mathsf{Prep}}
\newcommand{\Good}{\mathsf{Good}}
\newcommand{\Succ}{\mathsf{Succ}}
\newcommand{\init}{\mathsf{init}}
\newcommand{\TrapGen}{\mathsf{TrapGen}}
\newcommand{\td}{\mathsf{td}}


%\newcommand{\sid}{\mathsf{sid}}
%\newcommand{\commit}{\mathsf{commit}}

